Design-by-Contract for Flexible Multiparty Session Protocols -- Extended Version

Choreographic models support a correctness-by-construction principle in distributed programming. Also, they enable the automatic generation of correct message-based communication patterns from a global specification of the desired system behaviour. In this paper we extend the theory of choreography automata, a choreographic model based on finite-state automata, with two key features. First, we allow participants to act only in some of the scenarios described by the choreography automaton. While this seems natural, many choreographic approaches in the literature, and choreography automata in particular, forbid this behaviour. Second, we equip communications with assertions constraining the values that can be communicated, enabling a design-by-contract approach. We provide a toolchain allowing to exploit the theory above to generate APIs for TypeScript web programming. Programs communicating via the generated APIs follow, by construction, the prescribed communication pattern and are free from communication errors such as deadlocks.

==> Makefile <==
# title = "xyz" this should now be set by ~/bin/setlatex
LATEX = latexmk -f -latex="pdflatex --shell-escape"
BIBTEX = bibtex
TEX = main
host := $(shell hostname -s)

all:
	-$(LATEX) $(TEX).tex
	$(warning **** WARNINGS ****)
	grep Warning $(TEX).log

bib:
	$(BIBTEX) $(TEX)

e:
	e -T $(title) --reverse --no-splash -mm $(TEX).tex

onetex:
	latexpand -expand-bbl $(TEX).bbl $(TEX).tex > single_file.tex

clean:
	find . -name "*~" -exec rm -rf {} \;
	find . -name "*.log" -exec rm -rf {} \;
	find . -name "*.aux" -exec rm -rf {} \;
	find . -name "*.out" -exec rm -rf {} \;
	find . -name "*.synctex.gz" -exec rm -rf {} \;
	find . -name "*.bbl" -exec rm -rf {} \;
	find . -name "*.blg" -exec rm -rf {} \;
	find . -name "*.fdb*" -exec rm -rf {} \;
	find . -name "*.fls*" -exec rm -rf {} \;
	find . -name "*.axp*" -exec rm -rf {} \;
	find . -name "*.vtc*" -exec rm -rf {} \;

autorm:
	find . -name "auto" -exec rm -rf {} \;

show:
	pdfpc -p -g -z -e 15:10 $(NOTES).pdf



==> proofs.tex <==
\section{Proofs}

proofs

